Generating Natural Language Queries for More Effective Systematic Review Screening Prioritisation

Screening prioritisation in medical systematic reviews aims to rank the set of documents retrieved by complex Boolean queries. Prioritising the most important documents ensures that subsequent review steps can be carried out more efficiently and effectively. The current state of the art uses the final title of the review as a query to rank the documents using BERT-based neural rankers. However, the final title is only formulated at the end of the review process, which makes this approach impractical as it relies on ex post facto information. At the time of screening, only a rough working title is available, with which the BERT-based ranker performs significantly worse than with the final title. In this paper, we explore alternative sources of queries for prioritising screening, such as the Boolean query used to retrieve the documents to be screened and queries generated by instruction-based generative large-scale language models such as ChatGPT and Alpaca. Our best approach is not only viable based on the information available at the time of screening, but also has similar effectiveness to the final title.

==> table-generation-prompt.tex <==
\begin{table*}
\centering
\small
\begin{tabular}{@{}lll@{}}
\toprule
\bf Boolean Query & \bf Model: \bf Prompt & \bf Sample Output \\
\midrule
\multirow{2}{*}{\parbox[t]{245pt}{\raggedright\texttt{("Esophageal and Gastric Varices"[mesh:noexp] OR esophag* varic*[All Fields] OR esophag* varix[All Fields] OR esophago gastric varic*[All Fields] OR esophago gastric varix[All Fields] OR gastro esophag* varic*[All Fields] OR gastro esophag* varix[All Fields] OR gastro oesophag* varic*[All Fields] OR gastro oesophag* varix[All Fields] OR gastroesophag* varic*[All Fields] OR gastroesophag* varix[All Fields] OR gastrooesophag* varic*[All Fields] OR gastrooesophag* varix[All Fields] OR oesophag* varic*[All Fields] OR oesophag* varix[All Fields] OR oesophago gastric varic*[All Fields] OR oesophago gastric varix[All Fields] OR paraesophag* varic*[All Fields] OR paraesophag* varix[All Fields] OR paraoesophag* varic*[All Fields] OR paraoesophag* varix[All Fields] OR periesophag* varic*[All Fields] OR periesophag* varix[All Fields] OR perioesophag* varic*[All Fields] OR perioesophag* varix[All Fields])}\vskip-140pt}}
& 
\parbox[t]{150pt}{{\bf ChatGPT:} 
Construct a high-quality natural language query for the boolean query of a systematic review: \texttt{\{Boolean Query\}}.\\[0.25ex]
The effectiveness of the query will be determined by its capability to retrieve relevant documents when searching on a semantic-based search engine.}
& 
\parbox[t]{90pt}{What is the effectiveness of treatments for esophageal and gastric varices, including those related to esophag* varic* and gastroesophag* varic*?} 
\\
\cmidrule(l@{\tabcolsep}r@{\tabcolsep}){2-2}
& \parbox[t]{150pt}{{\bf Alpaca:} Below is an instruction that describes a task, paired with an input that provides further context. Write a response that appropriately completes the request.\\[0.25ex]
\#\#\# Instruction: 
Construct a natural language query using the systematic review boolean query provided. \\[0.25ex]
\#\#\# Input: 
\texttt{\{Boolean Query\}}\\[0.25ex]
\#\#\# Response:}
& \\
\bottomrule
\end{tabular}
\caption{ChatGPT's and Alpaca's Prompt and Sample Input/Output for converting a Boolean query into a natural language one.}
\label{table:generation_prompt}
\end{table*}

